A Simultaneous Dual-site Technosignature Search Using International LOFAR Stations

The Search for Extraterrestrial Intelligence aims to find evidence of technosignatures, which can point toward the possible existence of technologically advanced extraterrestrial life. Radio signals similar to those engineered on Earth may be transmitted by other civilizations, motivating technosignature searches across the entire radio spectrum. In this endeavor, the low-frequency radio band has remained largely unexplored; with prior radio searches primarily above 1 GHz. In this survey at 110-190 MHz, observations of 1,631,198 targets from TESS and Gaia are reported. Observations took place simultaneously with two international stations (noninterferometric) of the Low Frequency Array in Ireland and Sweden. We can reject the presence of any Doppler drifting narrowband transmissions in the barycentric frame of reference, with equivalent isotropic radiated power of 10 17 W, for 0.4 million (or 1.3 million) stellar systems at 110 (or 190) MHz. This work demonstrates the effectiveness of using multisite simultaneous observations for rejecting anthropogenic signals in the search for technosignatures.

==> rnaas.tex <==
% \documentclass[RNAAS]{aastex63}

% %% Define new commands here
% \newcommand\latex{La\TeX}
% \graphicspath{{./}{figures/}}
% \begin{document}

% \title{An example of a Research Note of the American Astronomical Society (RNAAS)}

% %% Note that the corresponding author command and emails has to come
% %% before everything else. Also place all the emails in the \email
% %% command instead of using multiple \email calls.
% \correspondingauthor{August Muench}
% \email{greg.schwarz@aas.org, august.muench@aas.org}

% \author{Ethan Vishniac}
% \altaffiliation{Editor-in-Chief}
% \affiliation{Johns Hopkins University}

% \author{Chris Lintott}
% \altaffiliation{RNAAS Editor}
% \affiliation{Oxford University}

% %% The \author command can take an optional ORCID.
% \author[0000-0002-0786-7307]{Greg J. Schwarz}
% \affiliation{American Astronomical Society \\
% 2000 Florida Ave., NW, Suite 300 \\
% Washington, DC 20009-1231, USA}

% \author{August Muench}
% \affiliation{American Astronomical Society \\
% 2000 Florida Ave., NW, Suite 300 \\
% Washington, DC 20009-1231, USA}

% %% Note that RNAAS manuscripts DO NOT have abstracts.
% %% See the online documentation for the full list of available subject
% %% keywords and the rules for their use.
% \keywords{editorials, notices --- 
% miscellaneous --- catalogs --- surveys}

% %% Start the main body of the article. If no sections in the 
% %% research note leave the \section call blank to make the title.
% \section{} 

% \textit{Research Notes of the \href{https://aas.org}{American Astronomical Society}}
% (\href{http://rnaas.aas.org}{RNAAS}) is a publication in the AAS portfolio
% (alongside ApJ, AJ, ApJ Supplements, and ApJ Letters) through which authors can 
% promptly and briefly share materials of interest with the astronomical community
% in a form that will be searchable via ADS and permanently archived.

% The astronomical community has long faced a challenge in disseminating
% information that may not meet the criteria for a traditional journal article.
% There have generally been few options available for sharing works in progress,
% comments and clarifications, null results, and timely reports of observations
% (such as the spectrum of a supernova), as well as results that wouldn’t
% traditionally merit a full paper (such as the discovery of a single exoplanet
% or contributions to the monitoring of variable sources). 

% Launched in 2017, RNAAS was developed as a supported and long-term
% communication channel for results such as these that would otherwise be
% difficult to broadly disseminate to the professional community and persistently
% archive for future reference.

% Submissions to RNAAS should be brief communications - 1,000 words or fewer
% \footnote{An easy way to count the number of words in a Research Note is to use
% the \texttt{texcount} utility installed with most \latex\ installations. The
% call  \texttt{texcount -incbib -v3 rnaas.tex}) gives 57 words in the front
% matter and 493 words in the text/references/captions of this template. Another
% option is by copying the words into MS/Word, and using ``Word Count'' under the
% Tool tab.}, and no more than a single figure (e.g. Figure \ref{fig:1}) or table
% (but not both) - and should be written in a style similar to that of a
% traditional journal article, including references, where appropriate, but not
% including an abstract.

% Unlike the other journals in the AAS portfolio, RNAAS publications are not
% peer reviewed; they are, however, reviewed by an editor for appropriateness
% and format before publication. If accepted, RNAAS submissions are typically
% published within 72 hours of manuscript receipt. Each RNAAS article is
% issued a DOI and indexed by ADS \citep{2000A&AS..143...41K} to create a
% long-term, citable record of work.

% Articles can be submitted in \latex\ (preferably with the new "RNAAS"
% style option in AASTeX v6.2), MS/Word, or via the direct submission in the
% \href{http://www.authorea.com}{Authorea} or
% \href{http://www.overleaf.com}{Overleaf} online collaborative editors.

% Authors are expected to follow the AAS's ethics \citep{2006ApJ...652..847K},
% including guidance on plagiarism \citep{2012AAS...21920404V}.

% %% An example figure call using \includegraphics
% \begin{figure}[h!]
% \begin{center}
% \includegraphics[scale=0.85,angle=0]{aas.pdf}
% \caption{Top page of the AAS Journals' website, \url{http://journals.aas.org},
% on October 15, 2017.  Each RNAAS manuscript is only allowed one figure or
% table (but not both). Including the
% \href{http://journals.aas.org//authors/data.html\#DbF}{data behind the figure}
% in a Note is encouraged, and the data will be provided as a link in the
% published Note.\label{fig:1}}
% \end{center}
% \end{figure}

% %% An example table using AASTeX's deluxetable. Note that since
% %% only one figure OR one table is allowed this is commented out.
% %\begin{deluxetable}{ccl}
% %\tablecaption{Example table some English and Greek letters\label{tab:1}}
% %\tablehead{
% %\colhead{Index number} & \colhead{English} & \colhead{Greek}
% %}
% %\startdata
% %1 & a & alpha ($\alpha$) \\
% %2 & b & beta ($\beta$) \\
% %3 & c & gamma ($\gamma$) \\
% %4 & d & delta ($\delta$) \\
% %5 & e & epsilon ($\epsilon$) \\
% %\enddata
% %\tablecomments{Long tables should only show a short example with the full
% %version as a machine readable table with the article.}
% %\end{deluxetable}  

% \acknowledgments

% Acknowledge people, facilities, and software here but remember that this counts
% against your 1000 word limit.

% \begin{thebibliography}{}

% \bibitem[Kennicutt et al.(2006)]{2006ApJ...652..847K} Kennicutt, R.~C., Jr., Vishniac, E., \& Sneden, C.\ 2006, \apj, 652, 847 

% \bibitem[Kurtz et al.(2000)]{2000A&AS..143...41K} Kurtz, M.~J., Eichhorn, G., Accomazzi, A., et al.\ 2000, \aaps, 143, 41 

% \bibitem[Vishniac(2012)]{2012AAS...21920404V} Vishniac, E.~T.\ 2012, American Astronomical Society Meeting Abstracts \#219, 219, 204.04 

% \end{thebibliography}

% \end{document}

